Enhancing Hyperedge Prediction with Context-Aware Self-Supervised Learning

Hypergraphs can naturally model group-wise relations (e.g., a group of users who co-purchase an item) as hyperedges. Hyperedge prediction is to predict future or unobserved hyperedges, which is a fundamental task in many real-world applications (e.g., group recommendation). Despite the recent breakthrough of hyperedge prediction methods, the following challenges have been rarely studied: (C1) How to aggregate the nodes in each hyperedge candidate for accurate hyperedge prediction? and (C2) How to mitigate the inherent data sparsity problem in hyperedge prediction? To tackle both challenges together, in this paper, we propose a novel hyperedge prediction framework (CASH) that employs (1) context-aware node aggregation to precisely capture complex relations among nodes in each hyperedge for (C1) and (2) self-supervised contrastive learning in the context of hyperedge prediction to enhance hypergraph representations for (C2). Furthermore, as for (C2), we propose a hyperedge-aware augmentation method to fully exploit the latent semantics behind the original hypergraph and consider both node-level and group-level contrasts (i.e., dual contrasts) for better node and hyperedge representations. Extensive experiments on six real-world hypergraphs reveal that CASH consistently outperforms all competing methods in terms of the accuracy in hyperedge prediction and each of the proposed strategies is effective in improving the model accuracy of CASH. For the detailed information of CASH, we provide the code and datasets at: https://github.com/yy-ko/cash.

==> files/eq3_CL.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.4\linewidth]{files/aux_legend.pdf}
\begin{tabular}{cccc}
    \centering
    \includegraphics[width=0.22\linewidth]{files/aux_citeseer.pdf}
     &  
    \includegraphics[width=0.22\linewidth]{files/aux_cora.pdf}
     &
    \includegraphics[width=0.216\linewidth]{files/aux_pubmed.pdf}
     &
    \includegraphics[width=0.216\linewidth]{files/aux_coraA.pdf}
     \\
    (a) {Citeseer}    
     & 
    (b) {Cora}
     &
    (c) {Pubmed}    
     & 
    (d) {Cora-A}
\end{tabular}
\caption{The impact of the dual contrative learning on the hyperedge prediction accuracy of {\m} according to the control hyperparameter $\beta$.
The auxiliary task is consistently beneficial to hyperedge prediction across a wide range of $\beta$ values.}\label{fig:eq3-contrastive}
\end{figure*}






==> files/eq4_efficiency.tex <==
\begin{figure*}[t]
\centering
\begin{tabular}{c}
\begin{tikzpicture}
\begin{axis}[
    % normalsize,
    height=4.5cm,
    ybar=5.5pt,
    bar width=10pt,
    width=0.95\linewidth,
    axis x line*=bottom,
    axis y line*=left,
    log origin=infty,
    % ybar=0,
    %bar width=4pt,
    % ymajorgrids,
    yminorticks=false,
    ymajorgrids,
    % enlarge x limits={abs=0.5cm},
    xlabel style={font=\footnotesize},
    ylabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize},
    ylabel={Training time (sec.)},%\\(sec. in log-scale)},
    ylabel style={align=center},
    % xlabel={Dataset},
    xlabel style={yshift=3pt,},
    ymin=0, ymax=100,
	symbolic x coords={Citeseer, Cora, Pubmed, Cora-A, DBLP-A, DBLP},
	xtick={Citeseer, Cora, Pubmed, Cora-A, DBLP-A, DBLP},
	% nodes near coords align=vertical,
	% clip=false,
    nodes near coords,
	legend style={at={(0.45,0.95)}, anchor=north, draw=},
	legend cell align=center,
	legend columns=4,
 	legend style={font=\small},
]
\addplot[font=\scriptsize, teal, pattern = north east lines, area legend, pattern color = teal, 	point meta=y,	visualization depends on=rawy\as\rawy,     ]
coordinates {
(Citeseer, 0.88)
(Cora, 0.76)
% (Pubmed, )
(Cora-A, 0.89)
% (DBLP-A, )
% (DBLP, )
};\addlegendentry{HyperSAGNN}

\addplot[font=\scriptsize, red, pattern = grid, area legend, pattern color = red, 	point meta=y,	visualization depends on=rawy\as\rawy,     ]
coordinates {
(Citeseer, 0.2)
(Cora, 0.3)
(Pubmed, 1.44)
(Cora-A, 0.2)
(DBLP-A, 4.01)
(DBLP, 4.02)
};\addlegendentry{NHP}


\addplot[font=\scriptsize, brown, pattern = vertical lines, area legend, pattern color = brown, 	point meta=y,	visualization depends on=rawy\as\rawy,     ]
coordinates {
(Citeseer, 2.2400)
(Cora, 2.9200)
(Pubmed, 22.66)
(Cora-A, 2.71)
(DBLP-A, 88.37)
(DBLP, 56.83)
};\addlegendentry{AHP}


\addplot[font=\scriptsize, blue, pattern = north west lines, area legend, pattern color = blue, 	point meta=y,	visualization depends on=rawy\as\rawy,     ]
coordinates {
(Citeseer, 2.0800)
(Cora, 3.0100)
(Pubmed, 19.7700)
(Cora-A, 2.1100)
(DBLP-A, 68.8200)
(DBLP, 57.0700)

};\addlegendentry{{\m}}
\end{axis}
\node[font=\scriptsize,color=teal,rotate=90] at (5.8, 0.38) {\textit{OOM}};
\node[font=\scriptsize,color=teal,rotate=90] at (11, 0.38) {\textit{OOM}};
\node[font=\scriptsize,color=teal,rotate=90] at (13.65, 0.38) {\textit{OOM}};
\end{tikzpicture}
\end{tabular}

\vspace{-3mm}
\caption{The average training time per epoch of hyperedge prediction methods on six real-world hypergraphs.}
\vspace{-4mm}
\label{fig:eq4-efficiency}
\end{figure*}


==> files/eq5_scalability.tex <==
\begin{figure*}[t]
\centering
\begin{tabular}{cccc}
    % \includegraphics[width=0.45\linewidth]{files/scale_citeseer.pdf}
     \begin{tikzpicture}
        \begin{axis}[
            width=0.25\linewidth,
            height=4cm,
            % grid
            grid=both,
            % grid style={line width=.1pt, draw=gray!10},
            major grid style={line width=.2pt,draw=gray!50},
            % x-axis
            xtick={0,0.2,0.4,0.6,0.8,1.0},
            xticklabels={0,0.2,0.4,0.6,0.8,1.0},
            xticklabel style ={font=},
            ylabel=Relative time, 
            xlabel=Ratio of hyperedges,
            ymin=0, ymax=11,
            xmin=0.0, xmax=1.1,
            ytick={0,2,4,6,8,10},
            yticklabels={0,2,4,6,8,10},
            xlabel style ={font=\small},
            ylabel style ={font=\small},
            yticklabel style ={font=\small},  
            ]
        % Citesser
        \addplot[color=blue,mark=triangle,line width=0.8pt]
        coordinates {(0.1,1)(0.2,1.94)(0.3,2.95)(0.4,3.95)(0.5,4.90)(0.6,5.81)(0.7,6.89)(0.8,7.63)(0.9,8.64)(1.0,10.05)};

        % linear
        \addplot[color=black!70,mark=None, dashed]
        coordinates {(0,0)(1.1,11)};
        \end{axis}
    \end{tikzpicture}

     &
     % \includegraphics[width=0.45\linewidth]{files/scale_cora.pdf}
     \begin{tikzpicture}
        \begin{axis}[
            width=0.25\linewidth,
            height=4cm,
            % grid
            grid=both,
            % grid style={line width=.1pt, draw=gray!10},
            major grid style={line width=.2pt,draw=gray!50},
            % x-axis
            xtick={0,0.2,0.4,0.6,0.8,1.0},
            xticklabels={0,0.2,0.4,0.6,0.8,1.0},
            xticklabel style ={font=},
            ylabel=Relative time, 
            xlabel=Ratio of hyperedges,
            ymin=0, ymax=11,
            xmin=0.0, xmax=1.1,
            ytick={0,2,4,6,8,10},
            yticklabels={0,2,4,6,8,10},
            xlabel style ={font=\small},
            ylabel style ={font=\small},
            yticklabel style ={font=\small},  
            ]
        
        % cora
        \addplot[color=blue,mark=triangle,line width=0.8pt]
        coordinates {(0.1,1)(0.2,2.10)(0.3,3.25)(0.4,4.34)(0.5,5.37)(0.6,6.44)(0.7,7.59)(0.8,8.58)(0.9,9.87)(1.0,10.83)};
        
        % linear
        \addplot[color=black!80,mark=None, dashed]
        coordinates {(0,0)(1.1,11)};
        \end{axis}
    \end{tikzpicture}

    & 

    \begin{tikzpicture}
        \begin{axis}[
            width=0.25\linewidth,
            height=4cm,
            % grid
            grid=both,
            % grid style={line width=.1pt, draw=gray!10},
            major grid style={line width=.2pt,draw=gray!50},
            % x-axis
            xtick={0,0.2,0.4,0.6,0.8,1.0},
            xticklabels={0,0.2,0.4,0.6,0.8,1.0},
            xticklabel style ={font=},
            ylabel=Relative time, 
            xlabel=Ratio of hyperedges,
            ymin=0, ymax=11,
            xmin=0.0, xmax=1.1,
            ytick={0,2,4,6,8,10},
            yticklabels={0,2,4,6,8,10},
            xlabel style ={font=\small},
            ylabel style ={font=\small},
            yticklabel style ={font=\small},  
            ]
        % Citesser
        \addplot[color=blue,mark=triangle,line width=0.8pt]
        coordinates {(0.1,1)(0.2,2.10)(0.3,3.32)(0.4,4.54)(0.5,5.95)(0.6,6.64)(0.7,7.9)(0.8,8.88)(0.9,10.22)(1.0,11.35)};

        % linear
        \addplot[color=black!70,mark=None, dashed]
        coordinates {(0,0)(1.1,11)};
        \end{axis}
    \end{tikzpicture}

     &
     % \includegraphics[width=0.45\linewidth]{files/scale_cora.pdf}
     \begin{tikzpicture}
        \begin{axis}[
            width=0.25\linewidth,
            height=4cm,
            % grid
            grid=both,
            % grid style={line width=.1pt, draw=gray!10},
            major grid style={line width=.2pt,draw=gray!50},
            % x-axis
            xtick={0,0.2,0.4,0.6,0.8,1.0},
            xticklabels={0,0.2,0.4,0.6,0.8,1.0},
            xticklabel style ={font=},
            ylabel=Relative time, 
            xlabel=Ratio of hyperedges,
            ymin=0, ymax=11,
            xmin=0.0, xmax=1.1,
            ytick={0,2,4,6,8,10},
            yticklabels={0,2,4,6,8,10},
            xlabel style ={font=\small},
            ylabel style ={font=\small},
            yticklabel style ={font=\small},  
            ]
        
        % cora
        \addplot[color=blue,mark=triangle,line width=0.8pt]
        coordinates {(0.1,1)(0.2,2.40)(0.3,3.52)(0.4,4.64)(0.5,5.65)(0.6,6.84)(0.7,7.9)(0.8,8.58)(0.9,10.04)(1.0,10.75)};
        
        % linear
        \addplot[color=black!80,mark=None, dashed]
        coordinates {(0,0)(1.1,11)};
        \end{axis}
    \end{tikzpicture}
        
     \\
     (a) {Citeseer}
     &
     (b) {Cora}
     &     
     (c) {DBLP-A}
     &
     (d) {DBLP}
\end{tabular}

\caption{The training time per epoch of {\m} with the increasing number of hyperedges. {\m} provides (almost) linear scalability with the increasing number of hyperedges.}\label{fig:eq4-scalability}



\end{figure*}
